HEAL-SWIN: A Vision Transformer On The Sphere

High-resolution wide-angle fisheye images are becoming more and more important for robotics applications such as autonomous driving. However, using ordinary convolutional neural networks or vision transformers on this data is problematic due to projection and distortion losses introduced when projecting to a rectangular grid on the plane. We introduce the HEAL-SWIN transformer, which combines the highly uniform Hierarchical Equal Area iso-Latitude Pixelation (HEALPix) grid used in astrophysics and cosmology with the Hierarchical Shifted-Window (SWIN) transformer to yield an efficient and flexible model capable of training on high-resolution, distortion-free spherical data. In HEAL-SWIN, the nested structure of the HEALPix grid is used to perform the patching and windowing operations of the SWIN transformer, enabling the network to process spherical representations with minimal computational overhead. We demonstrate the superior performance of our model on both synthetic and real automotive datasets, as well as a selection of other image datasets, for semantic segmentation, depth regression and classification tasks. Our code is publicly available at https://github.com/JanEGerken/HEAL-SWIN.

==> tags <==
!_TAG_EXTRA_DESCRIPTION	anonymous	/Include tags for non-named objects like lambda/
!_TAG_EXTRA_DESCRIPTION	fileScope	/Include tags of file scope/
!_TAG_EXTRA_DESCRIPTION	pseudo	/Include pseudo tags/
!_TAG_EXTRA_DESCRIPTION	subparser	/Include tags generated by subparsers/
!_TAG_FIELD_DESCRIPTION	epoch	/the last modified time of the input file (only for F\/file kind tag)/
!_TAG_FIELD_DESCRIPTION	file	/File-restricted scoping/
!_TAG_FIELD_DESCRIPTION	input	/input file/
!_TAG_FIELD_DESCRIPTION	name	/tag name/
!_TAG_FIELD_DESCRIPTION	pattern	/pattern/
!_TAG_FIELD_DESCRIPTION	typeref	/Type and name of a variable or typedef/
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_KIND_DESCRIPTION!BibTeX	B,booklet	/booklet/
!_TAG_KIND_DESCRIPTION!BibTeX	I,incollection	/incollection/
!_TAG_KIND_DESCRIPTION!BibTeX	M,mastersthesis	/mastersthesis/
!_TAG_KIND_DESCRIPTION!BibTeX	P,proceedings	/proceedings/
!_TAG_KIND_DESCRIPTION!BibTeX	a,article	/article/
!_TAG_KIND_DESCRIPTION!BibTeX	b,book	/book/
!_TAG_KIND_DESCRIPTION!BibTeX	c,conference	/conference/
!_TAG_KIND_DESCRIPTION!BibTeX	i,inbook	/inbook/
!_TAG_KIND_DESCRIPTION!BibTeX	j,inproceedings	/inproceedings/
!_TAG_KIND_DESCRIPTION!BibTeX	m,manual	/manual/
!_TAG_KIND_DESCRIPTION!BibTeX	n,misc	/misc/
!_TAG_KIND_DESCRIPTION!BibTeX	p,phdthesis	/phdthesis/
!_TAG_KIND_DESCRIPTION!BibTeX	s,string	/string/
!_TAG_KIND_DESCRIPTION!BibTeX	t,techreport	/techreport/
!_TAG_KIND_DESCRIPTION!BibTeX	u,unpublished	/unpublished/
!_TAG_KIND_DESCRIPTION!Sh	a,alias	/aliases/
!_TAG_KIND_DESCRIPTION!Sh	f,function	/functions/
!_TAG_KIND_DESCRIPTION!Sh	h,heredoc	/label for here document/
!_TAG_KIND_DESCRIPTION!Sh	s,script	/script files/
!_TAG_KIND_DESCRIPTION!Tex	B,bibitem	/bibliography items/
!_TAG_KIND_DESCRIPTION!Tex	C,command	/command created with \\newcommand/
!_TAG_KIND_DESCRIPTION!Tex	G,subparagraph	/subparagraphs/
!_TAG_KIND_DESCRIPTION!Tex	N,counter	/counter created with \\newcounter/
!_TAG_KIND_DESCRIPTION!Tex	P,paragraph	/paragraphs/
!_TAG_KIND_DESCRIPTION!Tex	b,subsubsection	/subsubsections/
!_TAG_KIND_DESCRIPTION!Tex	c,chapter	/chapters/
!_TAG_KIND_DESCRIPTION!Tex	e,environment	/environment created with \\newenvironment/
!_TAG_KIND_DESCRIPTION!Tex	i,xinput	/external input files/
!_TAG_KIND_DESCRIPTION!Tex	l,label	/labels/
!_TAG_KIND_DESCRIPTION!Tex	o,operator	/math operator created with \\DeclareMathOperator/
!_TAG_KIND_DESCRIPTION!Tex	p,part	/parts/
!_TAG_KIND_DESCRIPTION!Tex	s,section	/sections/
!_TAG_KIND_DESCRIPTION!Tex	t,theorem	/theorem created with \\newtheorem/
!_TAG_KIND_DESCRIPTION!Tex	u,subsection	/subsections/
!_TAG_OUTPUT_EXCMD	mixed	/number, pattern, mixed, or combineV2/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROC_CWD	/home/oscar/Work/Reseach/Papers/Heal-Swin-git/	//
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	5.9.0	/50ab7a73/
!_TAG_ROLE_DESCRIPTION!Sh!heredoc	endmarker	/end marker/
!_TAG_ROLE_DESCRIPTION!Sh!script	loaded	/loaded/
!_TAG_ROLE_DESCRIPTION!Tex!xinput	bibliography	/bibliography (.bib) file/
!_TAG_ROLE_DESCRIPTION!Tex!xinput	included	/external input file specified with \\include/
!_TAG_ROLE_DESCRIPTION!Tex!xinput	input	/external input file specified with \\input/
2005ApJ	cites.bib	/^@ARTICLE{2005ApJ...622..759G,$/;"	a
6296535	cites.bib	/^@ARTICLE{6296535,$/;"	a
7780721	cites.bib	/^@INPROCEEDINGS{7780721,$/;"	j
9913937	cites.bib	/^@ARTICLE{9913937,$/;"	a
Ablations	experiments.tex	/^\\paragraph{Ablations} To investigate how the model performance depends on the HEALPix-specific /;"	P	subsection:Experiments""Semantic segmentation of indoor fisheye images
Acknowledgments and Disclosure of Funding	acknowledgments.tex	/^\\section*{Acknowledgments and Disclosure of Funding}$/;"	s
Additional experiment: Spherical image classification	appendix_additional_experiments.tex	/^\\section{Additional experiment: Spherical image classification}$/;"	s
Additional results	appendix_model.tex	/^\\paragraph{Additional results}$/;"	P	subsection:Experimental details""Stanford 2D-3D-S experiments
Armeni2017Stanford	cites.bib	/^@ARTICLE{Armeni2017Stanford,$/;"	a
BarrowTenenbaum1977	cites.bib	/^@InProceedings{BarrowTenenbaum1977,$/;"	j
Cho2022SphericalTransformer	cites.bib	/^@article{Cho2022SphericalTransformer,$/;"	a
Classes and reweighting	appendix_model.tex	/^\\paragraph{Classes and reweighting} We adjust the number of output channels in the base HEAL-SW/;"	P	subsection:Experimental details""SynWoodscape and MNIST experiments
Computational complexity	appendix_model.tex	/^\\paragraph{Computational complexity}$/;"	P	subsection:Experimental details""Stanford 2D-3D-S experiments
Conclusion	conclusion.tex	/^\\section{Conclusion}$/;"	s
Dataset size ablation	experiments.tex	/^\\paragraph{Dataset size ablation} We also study the effects of the size of the dataset by train/;"	P	subsection:Experiments""Semantic segmentation of fisheye street scenes
Datasets	appendix_data.tex	/^\\section{Datasets}$/;"	s
Depth estimation	experiments.tex	/^\\subsection{Depth estimation}$/;"	u	section:Experiments
Dosovitskiy2021VisionTransformer	cites.bib	/^@inproceedings{Dosovitskiy2021VisionTransformer,$/;"	j
Experimental details	appendix_model.tex	/^\\section{Experimental details}$/;"	s
Experiments	experiments.tex	/^\\section{Experiments}$/;"	s
Fan2022SingelStrideSparseTransformer	cites.bib	/^@InProceedings{Fan2022SingelStrideSparseTransformer,$/;"	j
Guibas2022AdaptiveFourierNeuralOperators	cites.bib	/^@InProceedings{Guibas2022AdaptiveFourierNeuralOperators,$/;"	j
Guo2023SphericalWindowBasedPCTransformer	cites.bib	/^@InProceedings{Guo2023SphericalWindowBasedPCTransformer,$/;"	j
HEAL-SWIN	model.tex	/^\\section{HEAL-SWIN}$/;"	s
HEAL-SWIN	model.tex	/^\\subsection{HEAL-SWIN}$/;"	u	section:HEAL-SWIN
HEAL-SWIN versus SWIN for flat segmentation	appendix_model.tex	/^\\paragraph{HEAL-SWIN versus SWIN for flat segmentation}$/;"	P	subsection:Experimental details""SynWoodscape and MNIST experiments
Hardware and training details	appendix_model.tex	/^\\paragraph{Hardware and training details} $/;"	P	subsection:Experimental details""Stanford 2D-3D-S experiments
Hardware and training details	appendix_model.tex	/^\\paragraph{Hardware and training details} For the semantic segmentation task we train all model/;"	P	subsection:Experimental details""SynWoodscape and MNIST experiments
Hart2023Interpolated	cites.bib	/^@INPROCEEDINGS {Hart2023Interpolated,$/;"	j
He2021GaugeET	cites.bib	/^@inproceedings{He2021GaugeET,$/;"	j
Inference time	experiments.tex	/^\\paragraph{Inference time} $/;"	P	subsection:Experiments""Semantic segmentation of fisheye street scenes
Introduction	introduction.tex	/^\\section{Introduction}$/;"	s
Jiang20219SphericalCNNUnstructuredGrids	cites.bib	/^@InProceedings{Jiang20219SphericalCNNUnstructuredGrids,$/;"	j
Krachmalnicoff2019	cites.bib	/^@article{Krachmalnicoff2019,$/;"	a
Lai2022StratifiedTransformer	cites.bib	/^@InProceedings{Lai2022StratifiedTransformer,$/;"	j
Lai2023SphericalTransformer3DRecognition	cites.bib	/^@article{Lai2023SphericalTransformer3DRecognition,$/;"	a
Mao2021VoxelTransformer	cites.bib	/^@InProceedings{Mao2021VoxelTransformer,$/;"	j
Model architecture	appendix_model.tex	/^\\paragraph{Model architecture}$/;"	P	subsection:Experimental details""Stanford 2D-3D-S experiments
Patches and windows	model.tex	/^\\subsubsection{Patches and windows}$/;"	b	subsection:HEAL-SWIN""HEAL-SWIN
Real-world images	experiments.tex	/^\\subsubsection{Real-world images}$/;"	b	subsection:Experiments""Semantic segmentation of fisheye street scenes
Related work	related_work.tex	/^\\section{Related work}$/;"	s
Relative position bias	model.tex	/^\\subsubsection{Relative position bias}$/;"	b	subsection:HEAL-SWIN""HEAL-SWIN
Resolution	appendix_model.tex	/^\\paragraph{Resolution} In order to be close to the resolution used by HexRUNet~\\cite{zhang2019/;"	P	subsection:Experimental details""Stanford 2D-3D-S experiments
Resolution	appendix_model.tex	/^\\paragraph{Resolution} In order to eliminate resolution as a central parameter in comparing the/;"	P	subsection:Experimental details""SynWoodscape and MNIST experiments
Ruhling2022ClimFormer	cites.bib	/^@InProceedings{Ruhling2022ClimFormer,$/;"	j
Semantic segmentation of fisheye street scenes	experiments.tex	/^\\subsection{Semantic segmentation of fisheye street scenes}$/;"	u	section:Experiments
Semantic segmentation of indoor fisheye images	experiments.tex	/^\\subsection{Semantic segmentation of indoor fisheye images}$/;"	u	section:Experiments
Shifting	model.tex	/^\\subsubsection{Shifting} $/;"	b	subsection:HEAL-SWIN""HEAL-SWIN
Stanford 2D-3D-S	appendix_data.tex	/^\\paragraph{Stanford 2D-3D-S} The Stanford 2D-3D-Semantic dataset\\footnote{\\url{http:\/\/build/;"	P	section:Datasets
Stanford 2D-3D-S experiments	appendix_model.tex	/^\\subsection{Stanford 2D-3D-S experiments}$/;"	u	section:Experimental details
SynWoodscape and MNIST experiments	appendix_model.tex	/^\\subsection{SynWoodscape and MNIST experiments}$/;"	u	section:Experimental details
Synthetic images	experiments.tex	/^\\subsubsection{Synthetic images}$/;"	b	subsection:Experiments""Semantic segmentation of fisheye street scenes
The HEALPix grid	model.tex	/^\\subsection{The HEALPix grid}$/;"	u	section:HEAL-SWIN
The SWIN transformer	model.tex	/^\\subsection{The SWIN transformer}$/;"	u	section:HEAL-SWIN
Vaswani2017Attention	cites.bib	/^@inproceedings{Vaswani2017Attention,$/;"	j
WoodScape and SynWoodScape	appendix_data.tex	/^\\paragraph{WoodScape and SynWoodScape} For our experiments we use the WoodScape~\\cite{woodscap/;"	P	section:Datasets
Zonca2019	cites.bib	/^@article{Zonca2019,$/;"	a
\\confName	main.tex	/^\\def\\confName{CVPR}$/;"	C
\\confYear	main.tex	/^\\def\\confYear{2024}$/;"	C
\\emph	preamble.tex	/^\\renewcommand{\\emph}[1]{\\textit{#1}}$/;"	C
\\npatch	preamble.tex	/^\\newcommand{\\npatch}{n_{\\mathrm{patch}}}$/;"	C
\\npix	preamble.tex	/^\\newcommand{\\npix}{n_{\\mathrm{pix}}}$/;"	C
\\nshift	preamble.tex	/^\\newcommand{\\nshift}{n_{\\mathrm{shift}}}$/;"	C
\\nside	preamble.tex	/^\\newcommand{\\nside}{n_{\\mathrm{side}}}$/;"	C
\\nwindow	preamble.tex	/^\\newcommand{\\nwindow}{n_{\\mathrm{win}}}$/;"	C
\\paperID	main.tex	/^\\def\\paperID{15658} $/;"	C
\\rebuttal	preamble.tex	/^\\newcommand{\\rebuttal}[1]{#1}$/;"	C
\\recheight	graphics/class_colourbar.tex	/^\\newcommand{\\recheight}{0.2}$/;"	C
\\recspace	graphics/class_colourbar.tex	/^\\newcommand{\\recspace}{1.2}$/;"	C
\\recwidth	graphics/class_colourbar.tex	/^\\newcommand{\\recwidth}{\\recspace}$/;"	C
\\removed	preamble.tex	/^\\newcommand{\\removed}[1]{}$/;"	C
\\ybase	graphics/class_colourbar.tex	/^\\newcommand{\\ybase}{5.5}$/;"	C
\\ysep	graphics/class_colourbar.tex	/^\\newcommand{\\ysep}{0.4}$/;"	C
app:additional_experiments	appendix_additional_experiments.tex	/^\\label{app:additional_experiments}$/;"	l
app:datasets-details	appendix_data.tex	/^\\label{app:datasets-details}$/;"	l
app:flat_sem_seg_results	appendix_model.tex	/^\\label{app:flat_sem_seg_results}$/;"	l
app:heal-swin-model-details	appendix_model.tex	/^\\label{app:heal-swin-model-details}$/;"	l
bi2023	cites.bib	/^@article{bi2023,$/;"	a
carla17	cites.bib	/^@inproceedings{carla17,$/;"	j
cheng2019covariance	cites.bib	/^@article{cheng2019covariance,$/;"	a
cobb2021	cites.bib	/^@inproceedings{cobb2021,$/;"	j
cohen2018b	cites.bib	/^@inproceedings{cohen2018b,$/;"	j
cohen2019gauge	cites.bib	/^@inproceedings{cohen2019gauge,$/;"	j
defferrard2020	cites.bib	/^@inproceedings{defferrard2020,$/;"	j
driscoll1994	cites.bib	/^@article{driscoll1994,$/;"	a
duSphericalTransformerAdapting2021	cites.bib	/^@article{duSphericalTransformerAdapting2021,$/;"	a
eder2019convolutions	cites.bib	/^@inproceedings{eder2019convolutions,$/;"	j
esteves2018	cites.bib	/^@inproceedings{esteves2018,$/;"	j
esteves2020c	cites.bib	/^@inproceedings{esteves2020c,$/;"	j
extract_dependencies	find-latex-dependencies.sh	/^function extract_dependencies() {$/;"	f
fig:HEAL-SWIN	introduction.tex	/^    \\label{fig:HEAL-SWIN}$/;"	l
fig:best_stanford_pred	appendix_data.tex	/^    \\label{fig:best_stanford_pred}$/;"	l
fig:class_hists	appendix_data.tex	/^  \\label{fig:class_hists}$/;"	l
fig:dataset_ablation_HEALPix	experiments.tex	/^    \\label{fig:dataset_ablation_HEALPix}$/;"	l
fig:grid_shifting_scheme	model.tex	/^  \\label{fig:grid_shifting_scheme}$/;"	l
fig:half-sphere-image	appendix_data.tex	/^  \\label{fig:half-sphere-image}$/;"	l
fig:main_results	introduction.tex	/^    \\label{fig:main_results}$/;"	l
fig:pointcloud	experiments.tex	/^    \\label{fig:pointcloud}$/;"	l
fig:polar_gt_kept	appendix_data.tex	/^    \\label{fig:polar_gt_kept}$/;"	l
fig:polar_gt_removed	appendix_data.tex	/^    \\label{fig:polar_gt_removed}$/;"	l
fig:sample_predictions	experiments.tex	/^  \\label{fig:sample_predictions}$/;"	l
fig:shifting	model.tex	/^  \\label{fig:shifting}$/;"	l
fig:stanford_depth_sample	appendix_data.tex	/^    \\label{fig:stanford_depth_sample}$/;"	l
fig:stanford_rgb_sample	appendix_data.tex	/^    \\label{fig:stanford_rgb_sample}$/;"	l
fig:stanford_sample	appendix_data.tex	/^\\label{fig:stanford_sample}$/;"	l
fig:worst_legitimate_stanford_pred	appendix_data.tex	/^    \\label{fig:worst_legitimate_stanford_pred}$/;"	l
fig:worst_stanford_pred	appendix_data.tex	/^    \\label{fig:worst_stanford_pred}$/;"	l
fig:ws_problems	appendix_data.tex	/^  \\label{fig:ws_problems}$/;"	l
find_file_with_extension	find-latex-dependencies.sh	/^function find_file_with_extension() {$/;"	f
gerken2021geometric	cites.bib	/^@article{gerken2021geometric,$/;"	a
gerken2022	cites.bib	/^@inproceedings{gerken2022,$/;"	j
gorski1998analysis	cites.bib	/^@article{gorski1998analysis,$/;"	a
haim2019surface	cites.bib	/^@inproceedings{haim2019surface,$/;"	j
indoor	experiments.tex	/^\\label{indoor}$/;"	l
kannala2006	cites.bib	/^@article{kannala2006,$/;"	a
kondor2018	cites.bib	/^@inproceedings{kondor2018,$/;"	j
kurth2023	cites.bib	/^@inproceedings{kurth2023,$/;"	j
lam2022	cites.bib	/^@misc{lam2022,$/;"	n
leeSpherePHDApplyingCNNs2019	cites.bib	/^@article{leeSpherePHDApplyingCNNs2019,$/;"	a
liu2021Swin	cites.bib	/^@inproceedings{liu2021Swin,$/;"	j
liu2021swinv2	cites.bib	/^@inproceedings{liu2021swinv2,$/;"	j
nguyen2023a	cites.bib	/^@inproceedings{nguyen2023a,$/;"	j
perraudin2019	cites.bib	/^@article{perraudin2019,$/;"	a
pmlr-v139-shakerinava21a	cites.bib	/^@InProceedings{pmlr-v139-shakerinava21a,$/;"	j
process_file	find-latex-dependencies.sh	/^function process_file() {$/;"	f
ramachandran2021	cites.bib	/^@article{ramachandran2021,$/;"	a
sec:depth-estimation	experiments.tex	/^\\label{sec:depth-estimation}$/;"	l
sec:experiments	experiments.tex	/^\\label{sec:experiments}$/;"	l
sec:healpix	model.tex	/^\\label{sec:healpix}$/;"	l
sec:seg-real-world-images	experiments.tex	/^\\label{sec:seg-real-world-images}$/;"	l
sec:seg-synthetic-images	experiments.tex	/^\\label{sec:seg-synthetic-images}$/;"	l
sec:shifting	model.tex	/^\\label{sec:shifting}$/;"	l
sec:swin	model.tex	/^\\label{sec:swin}$/;"	l
sekkat2022	cites.bib	/^@article{sekkat2022,$/;"	a
subsec:sem_seg	experiments.tex	/^\\label{subsec:sem_seg}$/;"	l
swinunet	cites.bib	/^@InProceedings{swinunet,$/;"	j
tab:ablations	appendix_model.tex	/^  \\label{tab:ablations}$/;"	l
tab:computational	appendix_model.tex	/^\\label{tab:computational}$/;"	l
tab:flat_segmentation	appendix_results.tex	/^  \\label{tab:flat_segmentation}$/;"	l
tab:heal_swin_spatial_features	appendix_model.tex	/^    \\label{tab:heal_swin_spatial_features}$/;"	l
tab:inference_times	experiments.tex	/^    \\label{tab:inference_times}$/;"	l
tab:s2_mnist	appendix_additional_experiments.tex	/^  \\label{tab:s2_mnist}$/;"	l
tab:sem_seg_results	experiments.tex	/^\\label{tab:sem_seg_results}$/;"	l
tab:stanford_dataset	experiments.tex	/^  \\label{tab:stanford_dataset}$/;"	l
tab:stanford_dataset_acc_per_class	appendix_data.tex	/^  \\label{tab:stanford_dataset_acc_per_class}$/;"	l
tab:stanford_dataset_iou_per_class	appendix_data.tex	/^  \\label{tab:stanford_dataset_iou_per_class}$/;"	l
tab:stanford_heal_swin_spatial_features	appendix_model.tex	/^    \\label{tab:stanford_heal_swin_spatial_features}$/;"	l
tab:subset_classes	appendix_data.tex	/^  \\label{tab:subset_classes}$/;"	l
tatenoDistortionAwareConvolutionalFilters2018	cites.bib	/^@incollection{tatenoDistortionAwareConvolutionalFilters2018,$/;"	I
woodscape2019	cites.bib	/^@InProceedings{woodscape2019,$/;"	j
zhang2019b	cites.bib	/^@inproceedings{zhang2019b,$/;"	j

